Efficient Evolutionary Search Over Chemical Space with Large Language Models

Molecular discovery, when formulated as an optimization problem, presents significant computational challenges because optimization objectives can be non-differentiable. Evolutionary Algorithms (EAs), often used to optimize black-box objectives in molecular discovery, traverse chemical space by performing random mutations and crossovers, leading to a large number of expensive objective evaluations. In this work, we ameliorate this shortcoming by incorporating chemistry-aware Large Language Models (LLMs) into EAs. Namely, we redesign crossover and mutation operations in EAs using LLMs trained on large corpora of chemical information. We perform extensive empirical studies on both commercial and open-source models on multiple tasks involving property optimization, molecular rediscovery, and structure-based drug design, demonstrating that the joint usage of LLMs with EAs yields superior performance over all baseline models across single- and multi-objective settings. We demonstrate that our algorithm improves both the quality of the final solution and convergence speed, thereby reducing the number of required objective evaluations. Our code is available at http://github.com/zoom-wang112358/MOLLEO

==> tables/DST_2.tex <==

\begin{table}[]
\centering
\begin{tabular}{lcccc}
\toprule
                         & DST & MolLEO(MolSTM) & MolLEO(BioT5) & MolLEO(GPT-4) \\ \midrule
deco\_hop                & 0   & 0.599          & 0.613         & 0.827         \\ \midrule
drd2                     & 0   & 0.832          & 0.975         & 0.981         \\ \midrule
gsk3b                    & 0   & 0.702          & 0.898         & 0.889         \\ \midrule
qed                      & 0.939 & 0.937          & 0.937         & 0         \\ \bottomrule
\end{tabular}
\caption{Comparison between DST and \ours}
\label{tab:DST}
\end{table}

==> tables/ablations_operators_mini.tex <==
%\begin{tcolorbox}[breakable,colback=white,fontupper=\selectfont\scriptsize,tabularx={X||c|c|c|c}]
\begin{table}
\noindent\begin{minipage}{\textwidth}
\vspace{0.2cm}
\captionof{table}{Top-10 AUC on 5 random seeds for the JNK3 and perindopril\_mpo tasks using different combinations of genetic operators. 
}\label{tab:operatorabl}
\end{minipage}
\centering
{%
\begin{minipage}{0.7\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}
{l||c|c|c}
\toprule
\textbf{Operators}     & \clip     & \tfive    & \gpt      \\

\midrule
\suggest{}{
\makecell[l]{\textcolor{customblue}{\texttt{CROSSOVER}}: \\LLM\\
\textcolor{custompink}{\texttt{MUTATION}}: \\ Selected top $Y$ molecules,\\ mutated with LLM, pruned\\offspring by distance to\\top-1 molecule\\
} }    & \suggest{}{\makecell{peridopril\_mpo:\\0.490 ± 0.016 [linear] \\ 0.517 ± 0.006 [spherical]\\JNK3:\\0.692 ± 0.110 [linear]\\}}  &\suggest{}{\makecell{peridopril\_mpo:\\0.736 ± 0.014\\JNK3:\\0.429 ± 0.110\\}} &\suggest{}{\makecell{peridopril\_mpo:\\0.592 ± 0.035\\JNK3:\\0.794 ± 0.026\\}} \\
\bottomrule
%\end{tcolorbox}
\end{tabular}}
\end{minipage}
}

\end{table}

==> tables/additional_PMO.tex <==
\begin{table}[]
\renewcommand{\arraystretch}{1.1}

\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}cr|cccccc@{}}
\toprule
\makecell{Task type} & 
\makecell{Method\\objective ($\uparrow$)}  & REINVENT             & Graph GA    &   GP BO       & \makecell{\ours\\(MolSTM)} & \makecell{\ours\\(BioT5)} & \makecell{\ours\\(GPT-4)}                \\ \midrule
\multirow{9}{*}{\makecell{Name-based\\optimization}}
& \suggest{}{albuterol\_similarity} &\suggest{}{0.896 ± 0.008}&\suggest{}{0.874 ± 0.020}&\suggest{}{0.902 ± 0.019}&\suggest{}{\underline{0.929 ± 0.005}}&\suggest{}{\underline{0.968 ± 0.003}}&\suggest{}{\underline{\textbf{0.985 ± 0.024}}} \\
& \suggest{}{celecoxib\_rediscovery} &\suggest{}{\underline{0.716 ± 0.084}}&\suggest{}{0.582 ± 0.057}&\suggest{}{\underline{0.728 ± 0.048}}&\suggest{}{0.594 ± 0.105}&\suggest{}{0.508 ± 0.017}&\suggest{}{\underline{\textbf{0.864 ± 0.034}}} \\
& \suggest{}{troglitazone\_rediscovery} &\suggest{}{\underline{0.452 ± 0.048}}&\suggest{}{0.377 ± 0.010}&\suggest{}{\underline{0.405 ± 0.007}}&\suggest{}{0.381 ± 0.025}&\suggest{}{0.390 ± 0.044}&\suggest{}{\underline{\textbf{0.562 ± 0.019}}} \\
& \suggest{}{amlodipine\_mpo} &\suggest{}{0.642 ± 0.044}&\suggest{}{0.625 ± 0.040}&\suggest{}{0.552 ± 0.025}&\suggest{}{\underline{0.674 ± 0.018}}&\suggest{}{\underline{\textbf{0.776 ± 0.038}}}&\suggest{}{\underline{0.773 ± 0.037}} \\
& \suggest{}{fexofenadine\_mpo} &\suggest{}{0.769 ± 0.009}&\suggest{}{\underline{0.779 ± 0.025}}&\suggest{}{0.745 ± 0.009}&\suggest{}{\underline{0.789 ± 0.016}}&\suggest{}{0.773 ± 0.017}&\suggest{}{\underline{\textbf{0.847 ± 0.018}}} \\
& \suggest{}{osimertinib\_mpo} &\suggest{}{\underline{0.834 ± 0.046}}&\suggest{}{0.808 ± 0.012}&\suggest{}{0.762 ± 0.029}&\suggest{}{\underline{0.823 ± 0.007}}&\suggest{}{0.817 ± 0.016}&\suggest{}{\underline{\textbf{0.835 ± 0.024}}} \\
& \suggest{}{zaleplon\_mpo} &\suggest{}{0.347 ± 0.049}&\suggest{}{0.456 ± 0.007}&\suggest{}{0.272 ± 0.026}&\suggest{}{\underline{0.475 ± 0.018}}&\suggest{}{\underline{0.465 ± 0.026}}&\suggest{}{\underline{\textbf{0.510 ± 0.031}}} \\
& \suggest{}{median1} &\suggest{}{\underline{\textbf{0.372 ± 0.015}}}&\suggest{}{0.287 ± 0.008}&\suggest{}{0.325 ± 0.012}&\suggest{}{0.298 ± 0.019}&\suggest{}{\underline{0.338 ± 0.033}}&\suggest{}{\underline{0.352 ± 0.024}} \\
& \suggest{}{median2} &\suggest{}{\underline{0.294 ± 0.006}}&\suggest{}{0.229 ± 0.017}&\suggest{}{\underline{\textbf{0.308 ± 0.034}}}&\suggest{}{0.251 ± 0.031}&\suggest{}{0.259 ± 0.019}&\suggest{}{\underline{0.275 ± 0.045}} \\
\midrule
\multirow{2}{*}{\makecell{Structure-based\\optimization}}& \suggest{}{isomers\_c7h8n2o2} &\suggest{}{0.842 ± 0.029}&\suggest{}{\underline{0.949 ± 0.036}}&\suggest{}{0.662 ± 0.071}&\suggest{}{\underline{0.948 ± 0.036}}&\suggest{}{0.928 ± 0.038}&\suggest{}{\underline{\textbf{0.984 ± 0.008}}} \\
& \suggest{}{valsartan\_smarts} &\suggest{}{0.000 ± 0.000}&\suggest{}{0.000 ± 0.000}&\suggest{}{0.000 ± 0.000}&\suggest{}{0.000 ± 0.000}&\suggest{}{0.000 ± 0.000}&\suggest{}{\underline{\textbf{0.867 ± 0.092}}}\\
\midrule
&\multicolumn{1}{r|}{Total ($\uparrow$)} & \suggest{}{14.036}   & \suggest{}{13.823} &  \suggest{}{13.182}   & \suggest{}{14.557} & \suggest{}{15.424}&  \suggest{}{17.862}\\
&\multicolumn{1}{r|}{Rank ($\downarrow$)} & \suggest{}{4}   & \suggest{}{5} & \suggest{}{6}   & \suggest{}{3} & \suggest{}{2}&  \suggest{}{1}\\\bottomrule
\end{tabular}%
}
%\vspace{0.1cm}
\caption{Top-10 AUC of the additional 11 tasks from PMO. The best model for each task is bolded and the top three are underlined. We also report the sum of all tasks (total) and the rank of each model overall from all 23 tasks in PMO.}
\label{table:additionalPMO}
\end{table}

==> tables/multi-obj-table-dep.tex <==
\begin{sidewaystable}
\caption{Multi objective results. The best model for each task is bolded.} 
\label{table:multiobj}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}cc|cccc@{}}
\toprule
\multicolumn{2}{l|}{\makecell[l]{Task 1: maximize QED ($\uparrow$),\\minimize SA ($\downarrow$), maximize JNK3 ($\uparrow$)}}     & \makecell{Summation\\(Top-10 AUC) ($\uparrow$)} & Hypervolume ($\uparrow$) & Structural diversity ($\uparrow$) & Objective diversity ($\uparrow$)    \\ \midrule
\multicolumn{1}{c|}{\multirow{4}{*}{Summation}}        & Graph-GA        & 1.967 ± 0.088                    & 0.713 ± 0.083         & 0.741 ± 0.115  & 0.351 ± 0.079     \\
\multicolumn{1}{c|}{\multirow{4}{*}{}}        & \clip        & 2.177 ± 0.178                    &     0.625 ± 0.162   &  0.803 ± 0.011  &    \textbf{0.362 ± 0.074}   \\
\multicolumn{1}{c|}{}                                            & \tfive      & 1.946 ± 0.222                &   0.592 ± 0.199        & \textbf{0.805 ± 0.196}  &  0.341 ± 0.091   \\
\multicolumn{1}{c|}{}                                            & \gpt      & 2.367 ± 0.044                    & \textbf{0.752 ± 0.085}        & 0.726 ± 0.063  & 0.292  ± 0.076       \\ \midrule
\multicolumn{1}{c|}{\multirow{4}{*}{Pareto optimality}}         & Graph-GA        & 2.120 ± 0.159                             & 0.603 ± 0.082           & 0.761 ± 0.034    & 0.219 ± 0.117         \\
\multicolumn{1}{c|}{}                                            & \clip      &    2.234 ± 0.246              &     0.472 ± 0.248      &  0.739 ± 0.015  &   0.306 ± 0.085 \\
\multicolumn{1}{c|}{}                                            & \tfive      & 2.325 ± 0.164                &    0.630 ± 0.120       & 0.724 ± 0.020  & 0.339 ± 0.062    \\
\multicolumn{1}{c|}{}                                            & \gpt      & \textbf{2.482 ± 0.057}                             & 0.727 ± 0.038       & 0.745 ± 0.057   & 0.322 ± 0.104         \\ \midrule
\multicolumn{2}{l|}{\makecell[l]{Task 2: maximize QED ($\uparrow$),\\minimize SA ($\downarrow$), maximize GSKB3 ($\uparrow$)}}    &  &  &  & \\ \midrule
\multicolumn{1}{c|}{\multirow{4}{*}{Summation}}        & Graph-GA        & 2.186 ± 0.069                   & 0.719 ± 0.055           & 0.778 ± 0.122   & 0.379 ± 0.101        \\
\multicolumn{1}{c|}{\multirow{4}{*}{}}        & \clip        & 2.349 ± 0.132                    &  0.303 ± 0.024      &  \textbf{0.820 ± 0.010}  &  \textbf{0.440 ± 0.037}     \\
\multicolumn{1}{c|}{}                                            & \tfive      & 2.306 ± 0.120               &   0.693 ± 0.093        & 0.803 ± 0.013  & 0.384 ± 0.045    \\
\multicolumn{1}{c|}{}                                            & \gpt     & 2.543 ± 0.014                   & \textbf{0.832 ± 0.024}          & 0.715 ± 0.052    & 0.391 ± 0.021         \\ \midrule
\multicolumn{1}{c|}{\multirow{4}{*}{Pareto optimality}}         & Graph-GA        & 2.339 ± 0.139                             & 0.640 ± 0.034           & 0.816 ± 0.028   & 0.381 ± 0.071          \\
\multicolumn{1}{c|}{}                                            & \clip      &   2.340 ± 0.254               &     0.202 ± 0.054      & 0.770 ± 0.017   &  0.188 ± 0.010   \\
\multicolumn{1}{c|}{}                                            & \tfive      & 2.299 ± 0.203                &  0.645 ± 0.127         & 0.759 ± 0.022  & 0.371 ± 0.047    \\
\multicolumn{1}{c|}{}                                            & \gpt      & \textbf{2.631 ± 0.023}                             & 0.820 ± 0.024           & 0.646 ± 0.017   & 0.191 ± 0.026         \\ \midrule
\multicolumn{2}{c|}{\makecell[l]{Task 3: maximize QED ($\uparrow$), JNK3 ($\uparrow$),\\minimize SA ($\downarrow$), GSKB3 ($\downarrow$), DRD2 ($\downarrow$)}} &  &  &  &  \\ \midrule
\multicolumn{1}{c|}{\multirow{4}{*}{Summation}}        & Graph GA        & 3.856 ± 0.075                   & 0.162 ± 0.048         & 0.821 ± 0.024   & 0.226 ± 0.057     \\
\multicolumn{1}{c|}{\multirow{2}{*}{}}        & \clip        & 4.040 ± 0.097                    &   0.474 ± 0.193       &  0.783 ± 0.027  &    \textbf{0.413 ± 0.064}   \\
\multicolumn{1}{c|}{}                                            & \tfive      &  3.904 ± 0.092               & 0.266 ± 0.201          & \textbf{0.828 ± 0.005}  & 0.243 ± 0.081    \\
\multicolumn{1}{c|}{}                                            & \gpt      & 4.017 ± 0.048                   & 0.606 ± 0.086           & 0.726 ± 0.064   & 0.289 ± 0.050     \\ \midrule
\multicolumn{1}{c|}{\multirow{4}{*}{Pareto optimality}}         & Graph GA        & 4.051 ± 0.155                             & 0.606 ± 0.052         & 0.688 ± 0.047   & 0.294 ± 0.074         \\
\multicolumn{1}{c|}{}                                            & \clip      &   3.989 ± 0.145                &    0.381 ± 0.204       &  0.792 ± 0.030 &   0.258 ± 0.019  \\
\multicolumn{1}{c|}{}                                            & \tfive      & 3.946 ± 0.115                &  0.367 ± 0.177        & 0.784 ± 0.020  & 0.367 ± 0.177    \\
\multicolumn{1}{c|}{}                                            & \gpt      & \textbf{4.212 ± 0.034}                            & \textbf{0.696 ± 0.029}         & 0.641 ± 0.037   & 0.266 ± 0.062        \\ \bottomrule
\end{tabular}%
}

\end{sidewaystable}


==> tables/similaritybasedga_ablation.tex <==
\begin{table}[]
\centering
\caption{BioT5 seems to hurt the Graph GA results}
\begin{tabular}{@{}c|c@{}}
\toprule
                & JNK3         \\ \midrule
Graph GA without lm editing  & 0.742±0.068      \\
Graph GA + BioT5 & 0.728±0.079      \\ \bottomrule
\end{tabular}
\vspace{0.3cm}

\end{table}

==> tables/single-obj-table-full.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}c|ccccccccc@{}}
\toprule
\begin{tabular}[c]{@{}c@{}}Method\\ Assembly\end{tabular} & REINVENT             & Graph GA    & SELFIES-REINVENT & SMILES GA   & GP BO   & GPT-4    & \clip & \tfive & \gpt                 \\ \midrule
QED                                                       & 0.941±0.000          & 0.940±0.000 & 0.940±0.000      & 0.940±0.000 & 0.937±0.000  & 0.932±0.054 & 0.937±0.002      & 0.937±0.002&   \textbf{0.948±0.004}         \\
%SA                                                        & TBD                  & TBD         & TBD              & TBD         & TBD        & TBD  & TBD       & &            \\
%TPSA & \\
%plogp & \\
isomers\_c9h10n2o2pf2cl                                   & 0.642±0.054          & 0.719±0.047 & 0.733±0.029      & 0.860±0.065 & 0.469±0.180 & 0.873 ±0.048  & 0.871±0.039 &0.873±0.019  &  \textbf{0.874±0.053}  \\
JNK3                                                      & 0.783±0.023          & 0.553±0.136 & 0.631±0.064      & 0.316±0.022 & 0.564±0.155 & 0.583±0.042 & 0.643±0.226 &0.728±0.079 &  \textbf{0.790±0.027} \\
DRD2                                                      & 0.945±0.007          & 0.964±0.012 & 0.943±0.005      & 0.908±0.019 & 0.923±0.017  & 0.964±0.046       &   0.975±0.003     & \textbf{0.981±0.002}&    0.968±0.012        \\
GSK3$\beta$                                               & 0.865±0.043 & 0.788±0.070 & 0.780±0.037      & 0.629±0.044 & 0.851±0.041 & 0.492±0.075  & \textbf{0.898±0.0412} & 0.889±0.0145 &  0.863±0.047          \\
mestranol\_similarity                                     & 0.618±0.048          & 0.579±0.022 & 0.620±0.029      & 0.629±0.044 & 0.627±0.089 & 0.848±0.067 & 0.596±0.018 &0.717±0.104 &  \textbf{0.972±0.009} \\
thiothixene\_rediscovery                                  & 0.534±0.013          & 0.479±0.025 & 0.495±0.040      & 0.315±0.017 & 0.559±0.027 & 0.465±0.042 & 0.508±0.035& 0.696±0.081&  \textbf{0.727±0.052} \\
perindopril\_mpo                                          & 0.537±0.016          & 0.538±0.009 & 0.517±0.021      & 0.447±0.013 & 0.493±0.011 & 0.539±0.046 &0.558±0.045 & \textbf{0.737±0.020}&  0.600±0.031 \\
ranolazine\_mpo                                           & 0.760±0.009          & 0.728±0.012 & 0.748±0.018      & 0.699±0.026 & 0.735±0.013 & 0.597±0.082 & 0.725±0.040 &0.749±0.012 &  \textbf{0.769±0.022} \\
sitagliptin\_mpo                                          & 0.021±0.003          & 0.433±0.075 & 0.194±0.121      & 0.363±0.057 & 0.186±0.055 & 0.482±0.076 & 0.548±0.065 &0.506±0.100 &  \textbf{0.584±0.067} \\
deco\_hop                                                 & 0.666±0.044          & 0.619±0.004 & 0.631±0.012      & 0.611±0.006 & 0.629±0.018 & 0.782±0.046 & 0.613±0.016 &0.827±0.093 &  \textbf{0.942±0.013} \\
scaffold\_hop                                             & 0.560±0.019          & 0.517±0.007 & 0.525±0.013      & 0.494±0.011 & 0.548±0.019 & 0.678±0.088 & 0.527±0.019 & 0.559±0.102&  \textbf{0.971±0.004} \\ 
Total & \\
Rank & 4          & 0.517±0.007 & 0.525±0.013      & 0.494±0.011 & 0.548±0.019 & 5 & 3 & 2&  1\\\bottomrule
\end{tabular}%
}
\vspace{0.3cm}
\caption{Top-10 AUC of single objective results \yq{the value looks too small now, we should consider how to better present them, maybe we can drop 1-2 baselines? we can also note we select the top several methods to report from PMO here}}
\label{table:singleobj}
\end{table}

==> tables/small-multiobj-vertical.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}


\begin{wraptable}{r}{0.56\textwidth}
\large
\caption{\textbf{Summation and hypervolume scores of multi-objective results.} The best model for each task is bolded.}
\label{table:smallmultiobj}
  \centering
  \vspace{-10pt}
  \resizebox{0.52\textwidth}{!}{
  \begin{tabular}{@{}cc|cc@{}}
\toprule
\multicolumn{2}{l|}{\makecell[l]{Task 1: maximize QED ($\uparrow$),\\minimize SA ($\downarrow$), maximize JNK3 ($\uparrow$)}}     & \makecell{Summation\\(Top-10 AUC) ($\uparrow$)} & Hypervolume ($\uparrow$)     \\ \midrule
\multicolumn{1}{c|}{\multirow{4}{*}{Summation}}        & Graph-GA        & 1.967 ± 0.088                    & 0.713 ± 0.083             \\

\multicolumn{1}{c|}{\multirow{4}{*}{}}        & \clip        & 2.177 ± 0.178                    &     0.625 ± 0.162       \\
\multicolumn{1}{c|}{}                                            & \tfive      & 1.946 ± 0.222                &   0.592 ± 0.199            \\
\multicolumn{1}{c|}{}                                            & \gpt      & \textbf{2.367 ± 0.044}                    & \textbf{0.752 ± 0.085}                \\ \midrule
\multicolumn{1}{c|}{\multirow{4}{*}{Pareto optimality}}         & Graph-GA        & 2.120 ± 0.159                             & 0.603 ± 0.082                      \\
\multicolumn{1}{c|}{}                                            & \clip      &    2.234 ± 0.246              &     0.472 ± 0.248         \\
\multicolumn{1}{c|}{}                                            & \tfive      & 2.325 ± 0.164                &    0.630 ± 0.120             \\
\multicolumn{1}{c|}{}                                            & \gpt      & \textbf{2.482 ± 0.057}                             & \textbf{0.727 ± 0.038}                  \\ \midrule
\multicolumn{2}{l|}{\makecell[l]{Task 2: maximize QED ($\uparrow$),\\minimize SA ($\downarrow$), maximize GSKB3 ($\uparrow$)}}&  &  \\ \midrule
\multicolumn{1}{c|}{\multirow{4}{*}{Summation}}        & Graph-GA        & 2.186 ± 0.069                   & 0.719 ± 0.055                      \\
\multicolumn{1}{c|}{\multirow{4}{*}{}}        & \clip        & 2.349 ± 0.132                    &  0.303 ± 0.024             \\
\multicolumn{1}{c|}{}                                            & \tfive      & 2.306 ± 0.120               &   0.693 ± 0.093              \\
\multicolumn{1}{c|}{}                                            & \gpt     & \textbf{2.543 ± 0.014}                   & \textbf{0.832 ± 0.024}                       \\ \midrule
\multicolumn{1}{c|}{\multirow{4}{*}{Pareto optimality}}         & Graph-GA        & 2.339 ± 0.139                             & 0.640 ± 0.034                        \\
\multicolumn{1}{c|}{}                                            & \clip      &   2.340 ± 0.254               &     0.202 ± 0.054            \\
\multicolumn{1}{c|}{}                                            & \tfive      & 2.299 ± 0.203                &  0.645 ± 0.127               \\
\multicolumn{1}{c|}{}                                            & \gpt      & \textbf{2.631 ± 0.023}                             & \textbf{0.820 ± 0.024}                       \\ \midrule
\multicolumn{2}{c|}{\makecell[l]{Task 3: maximize QED ($\uparrow$), JNK3 ($\uparrow$),\\minimize SA ($\downarrow$), GSKB3 ($\downarrow$), DRD2 ($\downarrow$)}}& &  \\ \midrule
\multicolumn{1}{c|}{\multirow{4}{*}{Summation}}        & Graph GA        & 3.856 ± 0.075                   & 0.162 ± 0.048                 \\
\multicolumn{1}{c|}{\multirow{2}{*}{}}        & \clip        & \textbf{4.040 ± 0.097}                    &   0.474 ± 0.193                \\
\multicolumn{1}{c|}{}                                            & \tfive      &  3.904 ± 0.092               & 0.266 ± 0.201                \\
\multicolumn{1}{c|}{}                                            & \gpt      & 4.017 ± 0.048                   & \textbf{0.606 ± 0.086}                   \\ \midrule
\multicolumn{1}{c|}{\multirow{4}{*}{Pareto optimality}}         & Graph-GA        & 4.051 ± 0.155                             & 0.606 ± 0.052                     \\
\multicolumn{1}{c|}{}                                            & \clip      &   3.989 ± 0.145                &    0.381 ± 0.204         \\
\multicolumn{1}{c|}{}                                            & \tfive      & 3.946 ± 0.115                &  0.367 ± 0.177              \\
\multicolumn{1}{c|}{}                                            & \gpt      & \textbf{4.212 ± 0.034}                            & \textbf{0.696 ± 0.029}                   \\ \bottomrule
\end{tabular}%
}

\vspace{-10pt}
\end{wraptable}
